Robust Reinforcement Learning on State Observations with Learned Optimal Adversary

We study the robustness of reinforcement learning (RL) with adversarially perturbed state observations, which aligns with the setting of many adversarial attacks to deep reinforcement learning (DRL) and is also important for rolling out real-world RL agent under unpredictable sensing noise. With a fixed agent policy, we demonstrate that an optimal adversary to perturb state observations can be found, which is guaranteed to obtain the worst case agent reward. For DRL settings, this leads to a novel empirical adversarial attack to RL agents via a learned adversary that is much stronger than previous ones. To enhance the robustness of an agent, we propose a framework of alternating training with learned adversaries (ATLA), which trains an adversary online together with the agent using policy gradient following the optimal adversarial attack framework. Additionally, inspired by the analysis of state-adversarial Markov decision process (SA-MDP), we show that past states and actions (history) can be useful for learning a robust agent, and we empirically find a LSTM based policy can be more robust under adversaries. Empirical evaluations on a few continuous control environments show that ATLA achieves state-of-the-art performance under strong adversaries. Our code is available at https://github.com/huanzhang12/ATLA_robust_RL.

==> algo_adv_ppo_single.tex <==
\renewcommand{\thealgorithm}{}
\begin{algorithm}[htbp]
\caption{Alternating Training with Learned Adversaries (ATLA)}
\label{alg:adv_ppo}
\begin{algorithmic}[1]
\REQUIRE Environment $\mathcal{E}$, number of iterations $N_{iter}$, and batch size $B$.
\STATE{Initialize the agent's actor network $\pi(a|\hat{s})$ with parameters $\theta$.}
\STATE{Initialize the adversary's actor network $\nu(\hat{s}|s)$ with parameters $\phi$.}
\FOR{$i=1$ to $N_{iter}$}
%\STATE$\theta_i\leftarrow\theta_{i-1}$

\FOR{$j=1$ to $N_\pi$}
\STATE Run $\pi_\theta$ with fixed $\nu_\phi$ to collect a set of trajectories $\mathcal{D}_\pi:=\{(\hat{s}_{t}^{k,j}, a_{t}^{k,j}, r_{t}^{k,j}, \hat{s}_{t+1}^{k,j})\}\big\rvert_{k=1}^B$.
%\STATE $\{(s_{t}^{k,j}, \hat{s}_{t}^{k,j}, a_{t}^{k,j}, r_{t}^{k,j}, s_{t+1}^{k,j})\}\leftarrow\text{\textit{Adv\_Traj}}(\nu_{\phi},\pi_{\theta_{i-1}})$\COMMENT{\textit{Adv\_Traj} defined in Algorithm~\ref{alg:adversary}}
\STATE $\theta\leftarrow\text{PolicyOptimizer}(\mathcal{D}_\pi, \theta)$
\ENDFOR
%\STATE$\phi\leftarrow\phi_{i-1}$
\FOR{$j=1$ to $N_\nu$}
%\STATE Run $\pi_{\theta_{i}}\circ\nu_{\phi}$ to collect a set of trajectories $\mathcal{D}_j:=\{(s_{t}^{k,j}, \hat{s}_{t}^{k,j}, a_{t}^{k,j}, r_{t}^{k,j}, s_{t+1}^{k,j})\}\big\rvert_{k=1}^{N_{traj}}$.
% \STATE $\mathcal{D}\leftarrow\text{\textit{Adv\_Traj}}(\nu_{\phi},\pi_{\theta},B)$ \COMMENT{\textit{Adv\_Traj} defined in Algorithm~\ref{alg:adversary}}
\STATE Run $\nu_\phi$ with fixed $\pi_\theta$ to collect a set of trajectories $\mathcal{D}_\nu:=\{({s}_{t}^{k,j}, \hat{s}_{t}^{k,j}, -r_{t}^{k,j}, {s}_{t+1}^{k,j})\}\big\rvert_{k=1}^B$.
\STATE $\phi\leftarrow\text{PolicyOptimizer}(\mathcal{D}_\nu, \phi)$

\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> tables/bigtable_old.tex <==
\begin{table*}[tbh!]\centering
\caption{Average rewards $\pm$ standard deviation over 50 episodes on five baselines and SA-PPO~\citep{zhang2020robust}. We report natural rewards (no attacks) and rewards under six adversarial attacks, including a simple random noise attack, the critic based attack in~\citep{pattanaik2018robust}, MAD and RS attacks in~\cite{zhang2020robust}, Snooping attack proposed in~\cite{inkawhich2019snooping}, and the optimal attack proposed in this paper. In each row we bold the best (lowest) attack reward over all five attacks. The row for the most robust method is highlighted.}
\resizebox{\linewidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{Env.} & \multirow{2}{*}{\shortstack{$\ell_\infty$ norm perturb-\\ation budget $\epsilon$}}                                  & \multirow{2}{*}{Method} & \multirow{2}{*}{\shortstack{Natural\\ Reward}} & \multicolumn{6}{c|}{Attack Reward} & \multirow{2}{*}{\shortstack{Best\\ Attack}} \\
                      &                                                              &                         &                                   & Critic           & Random            & MAD       &      Snooping      & RS                    
                      & ``Optimal''
                      &  \\ \hline
                      &                                                              & PPO (vanilla)           &2554$\pm$853 & 1464 $\pm$523  & 2101$\pm$793  & 1410$\pm$ 655 & 2234$\pm$1103    &  794$\pm$238 &    \bf373$\pm$	9  &373\\
                      && SA-PPO~\citep{zhang2020robust}         &2234$\pm$	668 &  3789$\pm$	15 &2710$\pm$	801 & 2652$\pm$	835  &   2509$\pm$838  &  1130	$\pm$42&    \bf   751$\pm$	465&751\\
                      &     &   \citet{pattanaik2018robust}  &  2755$\pm$582   &   2681$\pm$	555  &  2265$\pm$	502  &  1395$\pm$337   &  1349$\pm$436    &  1219$\pm$	174   &  \bf 291$\pm$	7   &   291  \\
                      && ATLA-PPO (MLP)         & 2559	 $\pm$    958                &  3497$\pm$	556    &  2153$\pm$  882  &  1679$\pm$676    &  1769$\pm$562   &  2329$\pm$	870    &  \bf 976$\pm$	40  &     976  \\ 
                      && PPO (LSTM)         &  3060$\pm$       639.3             &  2705$\pm$ 986   &  2410$\pm$  786    &  2397$\pm$	905    &   2234$\pm$1103  &  811$\pm$ 74   &   \bf 784$\pm$	48 &784       \\ 
                      
                      && ATLA-PPO (LSTM)         & 3487$\pm$	452                     &  3524$\pm$	550    &  3474$\pm$ 401   &3081$\pm$	754      &   3130$\pm$692  &  1567$\pm$	347            & \bf 1224$\pm$	191 &  1224  \\ 
                      
                      
                      


\rowcolor{lightgray}\cellcolor{white}\multirow{-7}{*}{ Hopper}  &\cellcolor{white} \multirow{-7}{*}{0.075} &   ATLA-PPO (LSTM)+ SA Reg       &  3291$\pm$	600                    & 2073$\pm$	824     & 3165 $\pm$  576  &  2814$\pm$	725    &   2857$\pm$724  & 2244$\pm$	618             &   \bf 1455$\pm$	248  &   1455      \\ 
 \hline
                      &                                                              & PPO (vanilla)           & 3460 $\pm$ 1170                   & 3424 $\pm$ 1295   & 3007 $\pm$ 1200   & 2869 $\pm$ 1271   &  2786$\pm$962   & 1336 $\pm$ 654        &                \bf454$\pm$16  &  454         \\
                      && SA-PPO~\citep{zhang2020robust}         & 4775$\pm$	591                     &  4875$\pm$	30    & 4867$\pm$	39     &  3668$\pm$	1789    &  3928$\pm$1661   &  3808$\pm$	138    &    \bf 1723$\pm$	1555           &  1723     \\
                      &     &  \citet{pattanaik2018robust}  &   4058$\pm$	1410  &  4058$\pm$	1410   &  2840$\pm$	2018   &   2927$\pm$	1954  &  2568$\pm$2044   &   1713	$\pm$1807  &\bf733$\pm$	1012 &733   \\
                      && ATLA-PPO (MLP)         &  3138 $\pm$ 1061                    &  3243$\pm$	1004    & 3384  $\pm$ 1056  &  2596$\pm$	1005    &  2571$\pm$1084   &  3367$\pm$	1020    &  \bf 2213$\pm$	915  &    2213   \\ 
                      && PPO (LSTM)         &  2785$\pm$	1121                    &  2730$\pm$	1082    &  2578 $\pm$ 1007 &  2471$\pm$	1109    & 2286$\pm$1156    &  \bf 1259$\pm$	937    &  1523$\pm$	869 &      1259 \\ 
                      
                      && ATLA-PPO (LSTM)         & 3920$\pm$	129                     &  3915$\pm$	274    &3779  $\pm$  541  & 3963	 $\pm$  36  &  3716$\pm$666   &     \bf 3219 $\pm$   1132 &  3463$\pm$	1016  &      3219 \\ 

\rowcolor{lightgray}\cellcolor{white}\multirow{-7}{*}{Walker2d} & \cellcolor{white}\multirow{-7}{*}{0.05} & ATLA-PPO (LSTM)   +SA Reg      &  3842$\pm$	475                    & 3884$\pm$	132     &  3927$\pm$	368    & 3836$\pm$	492    &  3742$\pm$629   &  \bf 3239$\pm$	894    &   3676$\pm$	602 &    3239   \\  
\hline
                      &                                                              & PPO (vanilla)           &  5485		$\pm$    1160                 &  4934$\pm$	1022    &  5261$\pm$	1005     &  1759$\pm$	828    &   3668$\pm$547  &  268	$\pm$227          &            \bf-872	$\pm$ 436 &     -872   \\
                      &&SA-PPO~\citep{zhang2020robust}         &  5067$\pm$	695                    &  4805 $\pm$ 128   &  4986	$\pm$452    &  4662	$\pm$522    &  4079$\pm$768   &  3412	$\pm$1755    &      \bf 2511 $\pm$	1117  & 2511 \\
                      &     &   \citet{pattanaik2018robust}  &  3469$\pm$	1139   &  3469$\pm$	1139   &  2346$\pm$	459   &  1427$\pm$	625   &  1336$\pm$644   &   1289$\pm$	777  &  \bf-672$\pm$	100 & -672  \\
                      && ATLA-PPO (MLP)         &    4894$\pm$	123                &  4427$\pm$	104    &  4541 $\pm$ 691 & 1891$\pm$	885     &   2862$\pm$1137  &  842$\pm$	143    &  \bf33$\pm$327  &  33     \\ 
                      && PPO (LSTM)         &  5696	$\pm$  165                  &  5519	$\pm$ 114   & 5475	 $\pm$ 691 &  3800$\pm$  363    &   3723$\pm$1168  &  1069	$\pm$  382  &  \bf -513 $\pm$	104  &   -513    \\ 
                      
                      && ATLA-PPO (LSTM)         & 5612$\pm$	130                     &  5196	$\pm$ 134   & 5390 $\pm$  704  &  3903	$\pm$  217  &   4455$\pm$677  & 1096	 $\pm$  329  &  \bf 716$\pm$	256  &   716    \\ 
                      
\rowcolor{lightgray}\cellcolor{white}\multirow{-7}{*}{Ant} & \cellcolor{white}\multirow{-7}{*}{0.15} &  
ATLA-PPO (LSTM)     +SA Reg    &  5393	$\pm$139                    & 5295$\pm$	165     &  5366$\pm$	104    &  5240$\pm$	170    &   5135$\pm$413  &  4136$\pm$	149    &  \bf 3759$\pm$	112  &     3759  \\  
\hline
&                                                              & PPO (vanilla)           &  7112$\pm$	113                     &  5761$\pm$119    & 5486 $\pm$   1378  &  1836$\pm$	866     &  1637$\pm$843   &  489$\pm$   758       &  \bf -637$\pm$	267  &     -637   \\
        &&SA-PPO~\citep{zhang2020robust}         &  3635$\pm$	21                    & 3589$\pm$	21     &  3619$\pm$ 18   &  3624$\pm$	23    &   3616$\pm$21  &        3283$\pm$	20        &  \bf 3036	$\pm$17  &    3036   \\
        &     &  \citet{pattanaik2018robust}   &   5241$\pm$	1162  &  5440$\pm$	676   &  2910$\pm$	1694   & 1773$\pm$	1248   &  1465$\pm$726   &   1602$\pm$	1157  & \bf 447$\pm$	192  &  447\\
        && ATLA-PPO (MLP)         & 5417$\pm$	49                     &  5134$\pm$	38    & 5388 $\pm$ 34    &  4623	$\pm$1146    & 4167$\pm$1507    & \bf 2170$\pm$	2097     &  2709$\pm$	80  &     2170  \\ 
                      && PPO (LSTM)         & 5609$\pm$	98                     & 4294$\pm$	112     &  5395$\pm$ 158   &  4768$\pm$	106    &  4088$\pm$748  &  2899 $\pm$	2006 & \bf -886$\pm$	30             &     -886      \\ 
                      
                      && ATLA-PPO (LSTM)         & 5766 $\pm$    109                & 4008$\pm$	1031     & 5685 $\pm$   107 & 4807$\pm$ 	154    &   4906$\pm$182  &  3458$\pm$	1338            &  \bf 2485$\pm$	1488  &     2485  \\ 
                      
\rowcolor{lightgray}\cellcolor{white}\multirow{-7}{*}{HalfCheetah} & \cellcolor{white}\multirow{-7}{*}{0.15} & ATLA-PPO (LSTM)   +SA Reg      &  6300$\pm$	261                    & 5991$\pm$	209   &  6164$\pm$603   &  5790$\pm$	174       &   5785$\pm$671  &\bf 4806$\pm$	603              &  4971$\pm$ 357  &   4806    \\  
\hline
\end{tabular}
}
\label{tab:all_res}
\end{table*}

==> tables/opt_attack_table_old.tex <==
\begin{table*}[tb]\centering
\caption{Average episode rewards $\pm$ standard deviation over 50 episodes on PPO and SA-PPO models. We report natural rewards (no attacks) and rewards under six adversarial attacks, including a simple random noise attack, the critic based attack in \citet{pattanaik2018robust},MAD and RS attacks in \citet{zhang2020robust}, Snooping attack proposed in~\citet{inkawhich2019snooping}, and the optimal attack proposed in this paper. In each row we bold the best (lowest) attack reward over all five attacks. ``Optimal'' attack is better than other attacks in all environments, sometimes by a large margin.}%\textcolor{red}{Hongge: add snooping attack results here (we already have these results from main table?). Make sure to also check all texts and captions (there were some places mentioning we had five attacks, but now we have six). Please read the experiments section, including captions, once again.}}
\resizebox{\linewidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{Env.} & \multirow{2}{*}{\shortstack{$\ell_\infty$ norm perturb-\\ation budget $\epsilon$}}                                  & \multirow{2}{*}{Method} & \multirow{2}{*}{\shortstack{Natural\\ Reward}} & \multicolumn{6}{c}{Attack Reward}  \\
                      &                                                              &                         &                                   & Critic           & Random            & MAD &Snooping                     & RS                    
                      & “Optimal”
                      \\ \hline
                      &                                                              & PPO           &2554$\pm$853 & 1464 $\pm$523  & 2101$\pm$793  & 1410$\pm$ 655 & 2234$\pm$1103   &  794$\pm$238 &    \bf373$\pm$	9  \\
                      
                       
                      
                      
                      


\multirow{-2}{*}{ Hopper}  & \multirow{-2}{*}{0.075} & SA-PPO        &2234$\pm$	668 &  3789$\pm$	15 &2710$\pm$	801 & 2652$\pm$	835  & 2509$\pm$838   &  1130	$\pm$42&    \bf   751$\pm$	465    \\ 
 \hline
                      &                                                              & PPO           & 3460 $\pm$ 1170                   & 3424 $\pm$ 1295   & 3007 $\pm$ 1200   & 2869 $\pm$ 1271   &    2786$\pm$962& 1336 $\pm$ 654        &                \bf454$\pm$16           \\
                      
                      

\multirow{-2}{*}{Walker2d} & \multirow{-2}{*}{0.05} & SA-PPO        & 4775$\pm$	591                     &  4875$\pm$	30    & 4867$\pm$	39     &  3668$\pm$	1789    & 3928$\pm$1661   &  3808$\pm$	138    &    \bf 1723$\pm$	1555                \\
\hline
                      &                                                              & PPO           &  5485		$\pm$    1160                 &  4934$\pm$	1022    &  5261$\pm$	1005     &  1759$\pm$	828    &  3668$\pm$547  &  268	$\pm$227          &            \bf-872	$\pm$ 436    \\
                      
                      
                      
\multirow{-2}{*}{Ant} & \multirow{-2}{*}{0.15} &  
SA-PPO        &  5067$\pm$	695                    &  4805 $\pm$ 128   &  4986	$\pm$452    &  4662	$\pm$522    &  4079$\pm$768  &  3412	$\pm$1755    &      \bf 2511 $\pm$	1117   \\
\hline
&                                                              & PPO           &  7112$\pm$	113                     &  5761$\pm$119    & 5486 $\pm$   1378  &  1836$\pm$	866     &  1637$\pm$843  &  489$\pm$   758       &  \bf -637$\pm$	267     \\
        
                      
\multirow{-2}{*}{HalfCheetah} & \multirow{-2}{*}{0.15} & SA-PPO        &  3635$\pm$	21                    & 3589$\pm$	21     &  3619$\pm$ 18   &  3624$\pm$	23    &  3616$\pm$21  &        3283$\pm$	20        &  \bf 3036	$\pm$17    \\  
\hline
\end{tabular}
}
\label{tab:opt_attack}
\end{table*}

==> tables/robust_training_table_old.tex <==
\begin{table*}[tb]\centering
\caption{Average episode rewards $\pm$ standard deviation over 50 episodes on ATLA models and baselines. We report natural rewards (no attacks) and the best (lowest) attack rewards among six types of adversarial attacks, including a simple random noise attack, the critic based attack in~\citep{pattanaik2018robust}, MAD and RS attacks in~\cite{zhang2020robust}, Snooping attack proposed in~\cite{inkawhich2019snooping}, and the optimal attack proposed in this paper. For each environment, we bold the most robust model. Since both RS attack and our ``optimal'' attack are parameterized attacks, the ``best attack'' column represents the worst case agent performance \emph{under hundreds of adversaries}. See Appendix~\ref{sec:all_attack_results} for more details.}
\vspace{-1em}
\resizebox{0.85\linewidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{l|c|c|c|c|c}
\hline
\multirow{2}{*}{Env.} &  \multirow{2}{*}{\shortstack{State\\Dimension}}& \multirow{2}{*}{\shortstack{$\ell_\infty$ norm perturb-\\ation budget $\epsilon$}}                                  & \multirow{2}{*}{Method} & \multirow{2}{*}{\shortstack{Natural\\ Reward}} &  \multirow{2}{*}{\shortstack{Best\\ Attack}} \\
                      &&                                                              &                         &                            &  \\ \hline
                      &&                                                              & PPO (vanilla)           &2554$\pm$853 &373$\pm$	9\\
                      
                      &&& SA-PPO~\citep{zhang2020robust}        &2234$\pm$	668 & 751$\pm$	465\\
                      &&&   \citet{pattanaik2018robust} &  2755$\pm$582  &291$\pm$	7\\ 
                      &&& ATLA-PPO (MLP)         & 2559	 $\pm$    958                &      976$\pm$	40  \\ 
                      
                      &&& PPO (LSTM)         &  3060$\pm$       639.3             &784$\pm$	48      \\ 
                      
                      &&& ATLA-PPO (LSTM)         & 3487$\pm$	452                     &  1224$\pm$	191  \\ 
                      
                      
                      


\multirow{-6}{*}{ Hopper} & \multirow{-6}{*}{11}  & \multirow{-6}{*}{0.075} & \bf ATLA-PPO (LSTM)    +SA Reg     &  3291$\pm$	600                    & \bf 1455$\pm$	248     \\ 
 \hline
                      &&                                                              & PPO (vanilla)           & 3460 $\pm$ 1170                   &  454$\pm$16        \\
                      
                      &&& SA-PPO~\citep{zhang2020robust}         & 4775$\pm$	591                     &  1723$\pm$	1555     \\
                      &&     &  \citet{pattanaik2018robust}  &   4058$\pm$	1410  &733$\pm$	1012\\
                      &&& ATLA-PPO (MLP)         &  3138 $\pm$ 1061                    &    2213$\pm$	915   \\ 
                      
                      &&& PPO (LSTM)         &  2785$\pm$	1121                    &       1259$\pm$	937 \\ 
                      
                      &&& ATLA-PPO (LSTM)         & 3920$\pm$	129                     &     3219 $\pm$   1132 \\ 

\multirow{-6}{*}{Walker2d} & \multirow{-6}{*}{17}  & \multirow{-6}{*}{0.05} & \bf ATLA-PPO (LSTM)    +SA Reg     &  3842$\pm$	475                    &    \bf 3239$\pm$	894   \\  
\hline
                      &&                                                              & PPO (vanilla)           &  5485		$\pm$    1160                 &  -872	$\pm$ 436   \\
                      
                      &&& SA-PPO~\citep{zhang2020robust}         &  5067$\pm$	695                    & 2511 $\pm$	1117 \\
                      &  &   &   \citet{pattanaik2018robust}  &  3469$\pm$	1139   &-672$\pm$	100\\
                      &&& ATLA-PPO (MLP)         &    4894$\pm$	123                &  33$\pm$327     \\ 
                      
                      &&& PPO (LSTM)         &  5696	$\pm$  165                  &  -513 $\pm$	104    \\ 
                      
                      &&& ATLA-PPO (LSTM)          & 5612$\pm$	130                     &  716$\pm$	256    \\ 
                      
\multirow{-6}{*}{Ant} & \multirow{-6}{*}{111}  & \multirow{-6}{*}{0.15} &  
\bf ATLA-PPO (LSTM)     +SA Reg    &  5393$\pm$139                    &  \bf 3759$\pm$	112         \\  
\hline
&&                                                              & PPO (vanilla)           &  7112$\pm$	113                     &    -637$\pm$	267   \\

        &&& SA-PPO~\citep{zhang2020robust}         &  3635$\pm$	21                    &  3036	$\pm$17   \\
        &&     &  \citet{pattanaik2018robust}   &   5241$\pm$	1162  &447$\pm$	192\\
        &&& ATLA-PPO (MLP)         & 5417$\pm$	49                      &     2170$\pm$	2097  \\ 
        
                      &&& PPO (LSTM)         & 5609$\pm$	98                     &     -886$\pm$	30      \\ 
                      
                      &&& ATLA-PPO (LSTM)          & 5766 $\pm$    109                &   2485$\pm$	1488  \\ 
                      
\multirow{-6}{*}{HalfCheetah} & \multirow{-6}{*}{17}   & \multirow{-6}{*}{0.15} & \bf ATLA-PPO (LSTM)  +SA Reg       &  6300$\pm$	261                   &   \bf 4806$\pm$	603    \\  
\hline
\end{tabular}
}
\label{tab:rob_model_res}
\end{table*}
